Hard-Aware Deeply Cascaded Embedding

Riding on the waves of deep neural networks, deep metric learning has also achieved promising results in various tasks using triplet network or Siamese network. Though the basic goal of making images from the same category closer than the ones from different categories is intuitive, it is hard to directly optimize due to the quadratic or cubic sample size. To solve the problem, hard example mining which only focuses on a subset of samples that are considered hard is widely used. However, hard is defined relative to a model, where complex models treat most samples as easy ones and vice versa for simple models, and both are not good for training. Samples are also with different hard levels, it is hard to define a model with the just right complexity and choose hard examples adequately. This motivates us to ensemble a set of models with different complexities in cascaded manner and mine hard examples adaptively, a sample is judged by a series of models with increasing complexities and only updates models that consider the sample as a hard case. We evaluate our method on CARS196, CUB-200-2011, Stanford Online Products, VehicleID and DeepFashion datasets. Our method outperforms state-of-the-art methods by a large margin.

==> Makefile <==
# Copyright (c) 2008-2009 solvethis
# Copyright (c) 2010-2012 Casper Ti. Vector
# Public domain.

# 被编译的主文件的文件名，不包括扩展名。
JOBNAME = iccv_submit
# 这个变量的值可以为 latex、pdflatex 或 xelatex。
LATEX = pdflatex
# BIBTEX = biber -l zh__pinyin
DVIPDF = dvipdfmx

# 如果用 LaTeX 编译，则使用 dvipdfmx 将 dvi 转成 pdf。
ifeq ($(LATEX), latex)
	DODVIPDF = $(DVIPDF) $(JOBNAME)
endif

# 区分是 Windows 环境还是类 UNIX 环境。
# 如果是后者，则 GNU make 将可以检测到已经定义 PATH 环境变量。
ifdef PATH
	MAKE = make
	RM = rm -f
else
	MAKE = mingw32-make
	RM = del
endif

doc:
	$(LATEX) $(JOBNAME)
	$(BIBTEX) $(JOBNAME)
	$(LATEX) $(JOBNAME)
	$(LATEX) $(JOBNAME)
	# dvips -Ppdf -G0 -tletter iccv_submit.dvi
	# ps2pdf -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress iccv_submit.ps iccv_submit.pdf
	# $(BIBTEX) $(JOBNAME)
	# $(DODVIPDF)

clean:
	$(RM) $(JOBNAME).{aux,bbl,bcf,blg,dvi,lof,log,lot,run.xml,toc,out{,.bak}} \
		{missfont,texput}.log 

distclean: clean
	$(RM) $(JOBNAME).pdf

# vim:ts=4:sw=4

